Control-flow Flattening Preserves the Constant-Time Policy (Extended Version)

Obfuscating compilers protect a software by obscuring its meaning and impeding the reconstruction of its original source code. The typical concern when defining such compilers is their robustness against reverse engineering and the performance of the produced code. Little work has been done in studying whether the security properties of a program are preserved under obfuscation. In this paper we start addressing this problem: we consider control-flow flattening, a popular obfuscation technique used in industrial compilers, and a specific security policy, namely constant-time. We prove that this obfuscation preserves the policy, i.e., that every program satisfying the policy still does after the transformation.

==> sections/hoisting.tex <==

\subsection{Optimization: pre-computation/expression hoisting???}
\mnote{maybe just algebraic simplification?}
%
\begin{align*}
%    \hoist{\wop{+} \wemp} &= 0 \qquad \hoist{\wop{*} \wemp} = 1\\
  \hoist{\wop{+} \wlist{a_1}{\ldots}{a_n}} &=
        \begin{cases}
            v & \text{if } R = (v, \wemp)\\
            \wop{+} \wlist{b_1}{\ldots}{b_n} & \text{if } R = (0, \wlist{b_1}{\ldots}{b_m})\\
            \wop{+} \wlist{v}{b_1}{\ldots}{b_m}  & \text{if } R  = (v, \wlist{b_1}{\ldots}{b_m})
          \end{cases}\\
%          &\qquad \text{where } R = \aval{\wop{+} \wlist{\hoist{a_1}}{\ldots}{\hoist{a_n}}}\\
          % \aval{\wop{+} \wlist{a_1}\wlc
                                %\wlist{\hoist{a_1}}{\ldots}{\hoist{a_n}}}{\wemp}{0}\\
  \hoist{\wop{*} \wlist{a_1}{\ldots}{a_n}} &=
        \begin{cases}
          v & \text{if } R = (v, \wemp)\\
          0 & \text{if } R = (0, \wlist{b_1}{\ldots}{b_n})\\
            \wop{*} \wlist{b_1}{\ldots}{b_n} & \text{if } R = (1, \wlist{b_1}{\ldots}{b_n})\\
            \wop{*} \wlist{v}{b_1}{\ldots}{b_m}  & \text{if } R  = (v, \wlist{b_1}{\ldots}{b_m})
          \end{cases}\\
  %\aval{\wop{*} \wlist{\hoist{a_1}}{\ldots}{\hoist{a_n}}}{\wemp}{1}\\
  \hoist{\wop{-} a} &= \wop{-} \hoist{a} \\
  \hoist{a} &= a
\end{align*}
%
where $R = \aval{\wop{+} \wlist{\hoist{a_1}}{\ldots}{\hoist{a_n}}}$ and
$\aval{\cdot}$ inductively defined as follows:
\begin{align*}
  \aval{\wop{op}\wlist{v_1}{v_2}} &= (v_1 \mathrel{op} v_2, \wemp)   \\
  %
  \aval{\wop{op}\wlist{v}{a}} &= \aval{\wop{op}\wlist{a}{v}} = (v, \wlist{a}) \\
  %
  \aval{\wop{op}\wlist{a_1}{a_2}} &=  (\opunit, \wlist{a_1}{a_2}) \\
  %
  \aval{\wop{op} \wlist{v}{a_2}{\ldots}{a_n}} &= (v \mathrel{op} \pi_1(B), \pi_2(B))  \quad
                                           \text{ with } n > 2 \\
  %
  \aval{\wop{op} \wlist{a_1}{\ldots}{a_n}} &= (\pi_1(R),\wlist{a_1}\wlc \pi_2(B))
                                        \quad \text{ with } a_1 \notin \mb{N},  n > 2
\end{align*}
%
% \begin{align*}
%     \aval{\wop{op}\wlist{v_1}{v_2}}{\mi{il}}{t} &= \wop{op} (\wlist{(v_1 \mathrel{op} v_2) \mathrel{op} t} \wlc \mi{il}) \quad \mi{il} \neq \wemp   \\
%     \aval{\wop{op}\wlist{v}{a}}{\mi{il}}{t} &=  \aval{\wop{op}\wlist{a}{v}}{\mi{il}}{t} = \wop{op} (\wlist{v \mathrel{op} t}\wlc \wlist{a} \wlc \mi{il})    \quad \mi{il} \neq \wemp\\
%         \aval{\wop{op}\wlist{v_1}{v_2}}{\wemp}{t} &= (v_1 \mathrel{op} v_2) \mathrel{op} t  \\
%     \aval{\wop{op}\wlist{v}{a}}{\wemp}{t} &=  \aval{\wop{op}\wlist{a}{v}}{\wemp}{t} = \wop{op} (\wlist{v \mathrel{op} t}\wlc \wlist{a})  \quad v \mathrel{op} t \neq \mb{1}_{\mi{op}}\\
%         \aval{\wop{op}\wlist{v}{a}}{\wemp}{t} &=  \aval{\wop{op}\wlist{a}{v}}{\wemp}{t} = a   \quad v \mathrel{op} t = \mb{1}_{\mi{op}}\\
% %    \aval{\wop{op} \wemp}{\mi{il}}{t} &=
% %        \wop{op} (\wlist{t} \wlc \mi{il}) \text{ with } \mi{il} \neq \wemp\\
%     \aval{\wop{op} \wlist{v}{a_2}{\ldots}{a_n}}{\mi{il}}{t} &=
%         \aval{\wop{op} \wlist{a_2}{\ldots}{a_n}}{\mi{il}}{t \mathrel{op} v} \quad n > 2\\
%     \aval{\wop{op} \wlist{a_1}{\ldots}{a_n}}{\mi{il}}{t} &=
%         \aval{\wop{op} \wlist{a_2}{\ldots}{a_n}}{\wlist{a_1}\wlc\mi{il}}{t} \text{ with } a_1 \notin \mb{N},  n > 2\\
% \end{align*}
%
This function, given an expression $a$, returns a pair whose first element is the result of the computation and the
second one is the list of sub-expressions of $a$ that remains not evaluated.
Moreover, in the definition above $\opunit$ stands for the neutral element of $\mi{op}$;
$\cdot$ for the append on lists; $\src{B}$ for $\aval{\wop{op} \wlist{a_2}{\ldots}{a_n}}$; and
$\pi_i$ for the projection of the $i$th element of a tuple.

Similarly, we define a hoisting function for boolean expressions as follows:
%
\begin{align*}
    %\hoist{\wop{or} \wemp} &= \mtt{false}\\
    \hoist{\wop{or} \wlist{b_1}{\ldots}{b_n}} &= \bval{\wop{or} \wlist{\hoist{b_1}}{\ldots}{\hoist{b_n}}} \text{ with } n \geq 2\\
    \hoist{a_1 \wleq a_2} &= \bval{\hoist{a_1} \wleq \hoist{a_2}}\\
    \hoist{\wop{not} b} &= \wop{not} \hoist{b}
\end{align*}
%
where $\bval{\cdot}$ inductively defined as follows::
%
\begin{align*}
%    \bval{\wop{or} \mi{bl}}{\mi{il}}{\mtt{true}} &= \mtt{true}\\ %1
  \bval{\wop{or} \wlist{\mtt{true}}{b}} &= \bval{\wop{or} \wlist{b}{\mtt{true}}}
                                          = \mtt{true}\\ %3
  %
  \bval{\wop{or} \wlist{\mtt{false}}{b}} &= \bval{\wop{or}
                                           \wlist{b}{\mtt{false}}} = b\\
  %
  \bval{\wop{or} \wlist{b_1}{b_2}} &= \wop{or} \wlist{b_1}{b_2}
    \qquad\text{ with } b_1,b_2 \notin \{ \mtt{true}, \mtt{false}\}\\
  %                                             % 3
  \bval{\wop{or} \wlist{\mtt{false}}{b_2}{\ldots}{b_n}} &= \bval{\wop{or} \wlist{b_2}{\ldots}{b_n}} \text{ with } n > 2\\
  %
  \bval{\wop{or} \wlist{\mtt{true}}{b_2}{\ldots}{b_n}} &= \mtt{true} \text{ with } n > 2\\
  %
  \bval{\wop{or} \wlist{b_1}{\ldots}{b_n}} &=
  \begin{cases}
    \mtt{true} & \text{if } \bval{\wop{or} \wlist{b_2}{\ldots}{b_n}} = \mtt{true}\\
    b_1   & \text{if } \bval{\wop{or} \wlist{b_2}{\ldots}{b_n}} = \mtt{false}\\
    \wop{or} \wlist{b_1}\wlc ls & \text{if } \bval{\wop{or}
      \wlist{b_2}{\ldots}{b_n}} = ls \land b_1 \notin \{ \mtt{true}, \mtt{false}\}
  \end{cases}                                                &\qquad\qquad\qquad\qquad\text{ with }
                                                               n > 2 \\
  \bval{v_1 \leq v_2} &=
  \begin{cases}
    \mtt{true}  & \text{if } v_1 \leq v_2 \\
    \mtt{false} & \text{otherwise}
  \end{cases}\\
  \bval{a_1 \leq a_2} &= a_1 \leq a_2 \qquad a_1,a_2 \notin \mb{N}
\end{align*}
%

Finally, the hoisting definition for statements is:
%
\begin{align*}
  \hoist{\wskip} &= \wskip\\
  %
  \hoist{\wvar{x} \wassign a} &= \wvar{x} \wassign \hoist{a}\\
  %
  \hoist{c_1 \wseq c_2} &=\begin{cases}
                            \hoist{c_2} & \text{if } \hoist{c_1} = \wskip \\
                            \hoist{c_1} \wseq \hoist{c_2} & \text{otherwise}
                          \end{cases}\\
  %
  \hoist{\wif b \wthen c_1 \welse c_2 } &=\begin{cases}
                                            \hoist{c_1} & \text{if } \hoist{b} =
                                            \mtt{true} \\
                                            \hoist{c_2} & \text{if } \hoist{b} =
                                            \mtt{false} \\
                                            \wif \hoist{b} \wthen \hoist{c_1}
                                            \welse \hoist{c_2} & \text{otherwise}
                                          \end{cases}\\
  %
  \hoist{\wwhile b \wdo c} &=\begin{cases}
                               \wskip  & \text{if } \hoist{b} = \mtt{false} \\
                               \wwhile \hoist{b} \wdo \hoist{c} & \text{otherwise}
                             \end{cases}\\
  \hoist{\wswitch a : \wlist{(v_1, c_1)}{\ldots}{(v_n, c_n)}} &=
        \begin{cases}
             \hoist{c_i} &     \text{if } \exists i. \hoist{a} = v_i \\
             \wswitch \hoist{a} : \wlist{(v_1, \hoist{c_1})}{\ldots}{(v_n,
               \hoist{c_n})} & \text{otherwise}
        \end{cases}
\end{align*}
% \begin{align*}
%     \hoist{\wskip} &= \wskip\\
%     \hoist{\wvar{x} \wassign a} &= \wvar{x} \wassign \hoist{a}\\
%     \hoist{c_1 \wseq c_2} &= \hoist{c_1} \wseq \hoist{c_2}\\
%     \hoist{\wif b \wthen c_1 \welse c_2 } &= \wif \hoist{b} \wthen \hoist{c_1} \welse \hoist{c_2}\\
%     \hoist{\wwhile b \wdo c} &= \wwhile \hoist{b} \wdo \hoist{c}\\
%     \hoist{\wswitch a : \wlist{(v_1, c_1)}{\ldots}{(v_n, c_n)}} &= \wswitch \hoist{a} : \wlist{(v_1, \hoist{c_1})}{\ldots}{(v_n, \hoist{c_n})}
% \end{align*}
%


% \mnote{Ancora da sistemare la definizione. @Lillo: se hai voglia nella cartella trovi il file coq, dove c'è la formalizzazione per l'hoisting delle espressioni aritmetiche.}

\lnote{Scritto la definizione di hoist. Quella dei comandi è abbastanza
  aggressiva. C'è da capire se va in appendice. Una possibilità potrebbe mettere
tutto in una tabella}

\begin{example}[Hoisting breaks the \emph{step-counting} policy]
    \mnote{@Lillo: ti lascio la bozza dell'esempio qui -- dovremmo forse trovare una cosa più signifcativa, tipo il calcolo di una chiave...}
    Let $c$ be a program with a secret variable $x$ and that includes the fragment (for whatever reason):
    \begin{lstlisting}
        ...
        if x <= 3 then
            result = (21*x)+y
        else
            result = (8*3)+4
    \end{lstlisting}

    its optimized version is as follows
    \begin{lstlisting}
        ...
        if x <= 3 then
            result = (21*x)+y
        else
            result = 28
    \end{lstlisting}
    i.e., the program have a \emph{different} execution time depending on the secret value of $x$.
\end{example}

